ABot-3DWorld 0: A Universal World Model to Explore Any 3D Space

We present ABot-3DWorld 0, a universal multimodal 3D world model that turns text, image, and video inputs into high-fidelity, explorable 3D worlds. At the heart of our framework is a unified Spatial Generative Primitive (SGP), a compact tuple of a high-quality panorama and a spatial point cloud that delivers an efficient description of any 3D space. Multimodal inputs are first lifted into this primitive; a 3D-consistent panoramic video generator then explores the primitive along a planned trajectory; finally, our panoramic video reconstruction engine converts the generated video into a clean, photorealistic 3D Gaussian Splatting (3DGS) world. This pipeline covers two regimes: rich inputs (multi-view sets, casual video) are lifted into the SGP through a geometry-rigorous recovery that mirrors the observed scene, while a single image or sentence is completed generatively into a creative world. The result is one low-barrier engine for general 3D content creation that further anchors generated worlds to geographic points of interest, enabling map-native spatial exploration at consumer scale. Experiments show that ABot-3DWorld 0 sets the state of the art among open-source methods and demonstrates stronger scene fidelity than Marble under rich multimodal inputs.

==> sections/sec4_deployment.tex <==
\section{Deployment}
\label{sec:deployment}

Translating the algorithmic pipeline of \cref{sec:method} into a deployable product surface introduces engineering challenges that go well beyond a single research GPU. \method{} exposes two service tiers, \methodpro{} (quality-first) and \methodflash{} (latency-first), both backed by the same multi-stage acceleration strategy. This section outlines the key engineering choices.

\subsection{Acceleration Across the Pipeline}

\paragraph{Panoramic video generation}
The 14B VACE backbone is the dominant inference cost. We combine three orthogonal optimisations: (i) the LightX2V step distillation introduced in \cref{sec:method_video} reduces sampler cost by an order of magnitude; (ii) FlashAttention-3~\cite{hyworld22026} lowers per-step attention cost on Hopper GPUs; and (iii) sequence parallelism across multiple GPUs allows long panoramic sequences to be generated without splitting the spatial axis. The combination yields end-to-end panoramic video generation in well under 12 minute per scene on a typical 4-GPU 4090 nodes. For comparison, Hunyuan use four H20 with 20 minutes.  

\paragraph{3DGS reconstruction and FLUX repair}
We run the panoramic-SfM, 3DGS optimisation, and FLUX repair stages on a heterogeneous CPU--GPU mix. Multiple panoramic views are dispatched to GPU repair workers in parallel, while CPUs handle the lightweight Gaussian decimation and LOD generation. A scheduler tracks per-stage queues and load-balances repair tasks across GPUs to mitigate stragglers caused by scene complexity.

\paragraph{Renderer and asset delivery}
The trained 3DGS asset is exported into the standard 3D Tiles-compliant tileset together with our internal map-tile-path convention, allowing both the YunJing-based renderer and third-party 3D Tiles clients to consume the asset directly. A multi-resolution LOD organisation (zoom 14--19) is generated jointly with the asset, enabling smooth zoom-from-globe-to-room interaction at planet scale.

\subsection{Service Tiers}

\paragraph{ABot-3DWorld 0-Pro}
\methodpro{} prioritises generation quality. It runs the full panoramic generator at 1080p, applies the two-pass FLUX repair, and exports a multi-resolution 3DGS world with up to LOD-19 detail. Typical end-to-end latency from a single image is on the order of a few minutes on an 4-4090 nodes, comparable to the published latency of HY-World 2.0 / Marble while delivering markedly higher panoramic-texture fidelity.

\paragraph{ABot-3DWorld 0-Flash}
\methodflash{} is designed for a consumer-facing Spatial-TikTok feed, where the next world must be delivered in minutes. We trade off quality for latency along three dimensions: (i) the panoramic video resolution is reduced from 1080p to 720p, while model memory remains resident in VRAM via microserving to reduce loading overhead; (ii) the FLUX repair stage is reduced to a single pass over a subset of training views selected by farthest-point sampling over camera poses; and (iii) Gaussian splatting training uses SH degree = 0 together with a modified parallel FasterGS backend. We reuse the weights across reconstruction cycles to reduce the total number of iterations. On a 4×4090 node, the FLUX repair stage takes about 2 to 3 minutes, depending on the length of the selected views. The 3DGS training stage from sparse points takes about 1 minutes on a 4x4090 node.
\begin{table}[t]
    \centering
    \caption{Comparison of runtime and rental cost between \methodflash{} and Hunyuan.}
    \label{tab:rental_cost}
    \begin{tabular}{lcccc}
        \toprule
        Method & Hardware & Total Time & Cost per GPU-Hour & Total Cost \\
        \midrule
        \methodflash{} & 4$\times$4090 48GB & 25 min & 3 RMB/h & 6.0 RMB \\
        Hunyuan & 4 H20 GPUs & 32 min & 8 RMB/h & 17.1 RMB \\
        \bottomrule
    \end{tabular}
\end{table}
